Charged lepton flavour violation in muons: theory overview

We briefly overview some theoretical aspects of charged lepton flavour violation in rare muon transitions and decays. Relying on the effective field theory approach (model-independent), we discuss the probing power of charged lepton flavour violation processes regarding the new physics scale, especially in what concerns muon-electron conversion in nuclei. We then illustrate how these processes can provide valuable information (allowing to constrain, falsify - or conversely to learn about the underlying new physics properties) for a few examples of well-motivated extensions of the Standard Model. We finally comment on how leptonic CP violation should be carefully considered upon studies of charged lepton flavour violation in extensions of the Standard Model featuring heavy sterile fermions.

==> refs.tex <==
\bibitem{Crivellin:2017rmk}
A.~Crivellin, S.~Davidson, G.~M.~Pruna and A.~Signer,
%``Renormalisation-group improved analysis of $\mu\to e$ processes in a systematic effective-field-theory approach,''
JHEP \textbf{05} (2017), 117.
%[arXiv:1702.03020 [hep-ph]].

\bibitem{Davidson:2022nnl}
S.~Davidson and B.~Echenard,
%``Reach and complementarity of $\mu \rightarrow e$ searches,''
Eur. Phys. J. C \textbf{82} (2022) no.9, 836.
%[arXiv:2204.00564 [hep-ph]].

\bibitem{Heeck:2022wer}
J.~Heeck, R.~Szafron and Y.~Uesaka,
%``Isotope dependence of muon-to-electron conversion,''
Nucl. Phys. B \textbf{980} (2022), 115833.
%[arXiv:2203.00702 [hep-ph]].

\bibitem{Calibbi:2017uvl}
L.~Calibbi and G.~Signorelli,
%``Charged Lepton Flavour Violation: An Experimental and Theoretical Introduction,''
Riv. Nuovo Cim. \textbf{41} (2018) no.2, 71-174.
%[arXiv:1709.00294 [hep-ph]].

\bibitem{Alvarez:2023dzz}
A.~Alvarez, A.~Banik, R.~Cepedello, B.~Herrmann, W.~Porod, M.~Sarazin and M.~Schnelke,
%``Accommodating muon (g \ensuremath{-} 2) and leptogenesis in a scotogenic model,''
JHEP \textbf{06} (2023), 163.
%[arXiv:2301.08485 [hep-ph]].

\bibitem{Calibbi:2022wko}
L.~Calibbi and X.~Gao,
%``Lepton flavor violation in minimal grand unified type II seesaw models,''
Phys. Rev. D \textbf{106} (2022) no.9, 095036.
%[arXiv:2206.10682 [hep-ph]].

\bibitem{Kriewald:2022erk}
J.~Kriewald, J.~Orloff, E.~Pinsard and A.~M.~Teixeira,
%``Prospects for a flavour violating $Z^\prime $ explanation of $\Delta a_{\mu ,e}$,''
Eur. Phys. J. C \textbf{82} (2022) no.9, 844.
%[arXiv:2204.13134 [hep-ph]].

\bibitem{Abada:2021zcm}
A.~Abada, J.~Kriewald and A.~M.~Teixeira,
%``On the role of leptonic CPV phases in cLFV observables,''
Eur. Phys. J. C \textbf{81} (2021) no.11, 1016.
%[arXiv:2107.06313 [hep-ph]].

\bibitem{Abada:2022asx}
A.~Abada, J.~Kriewald, E.~Pinsard, S.~Rosauro-Alcaraz and A.~M.~Teixeira,
%``LFV Higgs and Z-boson decays: leptonic CPV phases and CP asymmetries,''
Eur. Phys. J. C \textbf{83} (2023) no.6, 494.
%[arXiv:2207.10109 [hep-ph]].

\bibitem{Abada:2023raf}
A.~Abada, J.~Kriewald, E.~Pinsard, S.~Rosauro-Alcaraz and A.~M.~Teixeira,
``Heavy neutral lepton corrections to SM boson decays: lepton flavour universality violation in low-scale seesaw realisations,''
arXiv:2307.02558 [hep-ph].
